Learning to Make Analogies by Contrasting Abstract Relational Structure

Analogical reasoning has been a principal focus of various waves of AI research. Analogy is particularly challenging for machines because it requires relational structures to be represented such that they can be flexibly applied across diverse domains of experience. Here, we study how analogical reasoning can be induced in neural networks that learn to perceive and reason about raw visual data. We find that the critical factor for inducing such a capacity is not an elaborate architecture, but rather, careful attention to the choice of data and the manner in which it is presented to the model. The most robust capacity for analogical reasoning is induced when networks learn analogies by contrasting abstract relational structures in their input domains, a training method that uses only the input data to force models to learn about important abstract features. Using this technique we demonstrate capacities for complex, visual and symbolic analogy making and generalisation in even the simplest neural network architectures.

==> Acknowledgments.tex <==
\textbf{Acknowledgments}

Fabio Viola, János Kramár


==> experiments.tex <==
\clearpage

\section{Experiments}

\begin{table}[]
\begin{tabular}{@{}lll@{}}
{\ul \textbf{}} & Rigid relations & Fluid relations \\ \midrule
\multicolumn{1}{|l|}{\textbf{Relation}} & \multicolumn{1}{l|}{\textbf{Training Attribute}} & \multicolumn{1}{l|}{\textbf{Training Attributes}} \\ \midrule
\multicolumn{1}{|l|}{PROG} & \multicolumn{1}{l|}{\texttt{color-of-shape}} & \multicolumn{1}{l|}{\scriptsize{\texttt{\begin{tabular}[c]{@{}l@{}}color-of-shape, color-of-line,\\ size-of-shape, number-of-shape, \\ type-of-shape\end{tabular}}}} \\ \midrule
\multicolumn{1}{|l|}{XOR} & \multicolumn{1}{l|}{\texttt{color-of-shape}} & \multicolumn{1}{l|}{\scriptsize{\texttt{\begin{tabular}[c]{@{}l@{}}color-of-shape, color-of-line,\\ size-of-shape, position-of-shape, \\ type-of-shape\end{tabular}}}} \\ \midrule
\multicolumn{1}{|l|}{OR} & \multicolumn{1}{l|}{\texttt{color-of-shape}} & \multicolumn{1}{l|}{\scriptsize{\texttt{\begin{tabular}[c]{@{}l@{}}color-of-shape, color-of-line,\\ size-of-shape, position-of-shape, \\ type-of-shape\end{tabular}}}} \\ \midrule
\multicolumn{1}{|l|}{AND} & \multicolumn{1}{l|}{\texttt{color-of-shape}} & \multicolumn{1}{l|}{\scriptsize{\texttt{\begin{tabular}[c]{@{}l@{}}color-of-shape, color-of-line,\\ size-of-shape, position-of-shape, \\ type-of-shape\end{tabular}}}} \\ \bottomrule
\end{tabular}
\caption{The rigid and fluid relations conditions applied in training the \texttt{progression (PROG), XOR, OR} and \texttt{AND} relations in Experiment 1. In each case models are tested on applying the four relations with the attribute \texttt{type-of-line}.}
\label{my-label}
\end{table}


\begin{itemize}
    \item What is analogy?
    \item Why is it important?
    \item Who and how has it been studied (neuro, AI)
\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=0.475\textwidth]{./figures/perceptual_vs_semantic_candidates.pdf}
    \caption{The perceptually-plausible vs. semantically-plausible answer candidate conditions in Experiment 1. Perceptually plausible candidates involve variation in the same attribute as the correct answer (and thus have visual properties in common). Semantically plausible candidates are constructed by applying plausible but incorrect relations to the second row of the analogy question.}
    \label{fig:rpm_intro}
\end{figure}



==> rpm.tex <==
\newpage
\section{Applying analogy in more complex reasoning problems}

\david{Experiments currently running!}

Visual IQ tests are widely used for measuring human abstract reasoning ability. These tests usually contain difficult analogical reasoning problems, so they provide a useful measurement of analogical reasoning in neural networks. In particular, an abstract reasoning dataset inspired by a well known human-IQ test \cite{raven1938raven} was recently developed \cite{barretthillsantoro18}. This dataset, called the \emph{Procedurally Generated Matrices} (PGM) dataset is publically available online\footnote{Abstract reasoning dataset https://github.com/deepmind/abstract-reasoning-matrices}. 

Similar to our analogical reasoning dataset in section 1, the PGM dataset contains a wide variety of multiple-choice abstract reasoning problems. Each problem is presented as a 3x3 matrix of panels with one panel missing. The task is to complete the matrix by choosing a panel from a set of 8 multiple choice candidates. The correct panel must be chosen to satisfy some relation that exists between the panels. Many of these matrix problems measure analogical reasoning. To choose the correct panel, a test-taker must identify a relation across a row (or column) and then reapply this relation across the final row (or column). This dataset also tests various forms of generalization. For most of these generalization tests, current methods fail to learn abstract reasoning solutions that generalize.

We attempt to improve abstract reasoning generalistion using LBC. The current state-of-the-art models for the PGM dataset calculate a score for each multiple choice candidate, by inserting the candidate into the matrix and computing a score value for that matrix completion by passing the matrix images through a neural network. Since there are eight panels, there will be eight scores, each produced by the same neural network. To use LBC, instead of generating a set of semantically plausible multiple choice candidates, we instead use the scores produced by the network to select the k candidates with the highest scores. Instead of using all multiple choice candidates for training, we only used the k candidates with the highest scores, along with the score of the correct candidate. In this way, we are learning by contrasting, only using the most plausible alternative candidates, as determined by the neural network itself.

We find ...

Table with RPM results:\\ 
(i) neutral splits and generalisation splits, as in ICML paper.\\
(ii) top-K training\\
(iii) 'clever candidate' training\\
(iv) 'random candidate' training

% We impliment the Wild-Resnet described in \cite{barretthillsantoro18}. 



